General existence of minimal surfaces of genus zero with catenoidal ends and prescribed flux

For each end of complete minimal surface in the Euclidean 3-space, the flux vector is defined. It is well-known that the sum of the flux vector over all ends are zero. Consider the following inverse problem: For each balanced n-vectors, find an n-end catenoid which realizes these vectors as flux. Here, an n-end catenoid is a complete minimal surface of genus zero with ends asymptotic to the catenoids. In this paper, we show that the inverse problem can be solved for almost all balanced n vectors for arbitrary n, which is grater than 4. The assumption "almost all" is needed because nonexistence is known for special balanced vectors. We remark that in the case of n=4, the same result has been obtained by the authors (dg-ga/9709006). And the case n=3 is treated by Lopez and Berbanel.

==> macros.tex <==
\makeatletter
\def\eqncases#1{\stepcounter{equation}\let\@currentlabel=\theequation
 \global\@eqnswtrue\global\@eqcnt\z@\tabskip0pt%%\tabskip\@centering
 \let\\=\@eqncr
 $$\rightline\bgroup\noindent$
 \left\{\,\vcenter\bgroup
 \halign to #1\displaywidth \bgroup\@eqnsel\hskip\@centering
   $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne 
   \hskip 2\arraycolsep \hfil${##}$\hfil
   &\global\@eqcnt\tw@ \hskip 2\arraycolsep 
   $\displaystyle\tabskip\z@{##}$\hfil\tabskip\@centering
   &\llap{##}\tabskip\z@\cr}
\def\endeqncases{\@@eqncr\egroup
      \global\advance\c@equation\m@ne\egroup\right.$
      \egroup$$\global\@ignoretrue}
\let\@seqncr=\@eqncr
\@namedef{eqncases*}{\def\@eqncr{\nonumber\@seqncr}\eqncases}
\@namedef{endeqncases*}{\nonumber\endeqncases}
\makeatother



%%%%%%%%%%%%%%%%%%NewCommand%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{{\bf C}}
\newcommand{\R}{{\bf R}}
\newcommand{\K}{{\bf K}}
\newcommand{\Z}{{\mbox{Z}}}
\newcommand{\Q}{{\bf Q}}
\newcommand{\hatC}{{\bf C}\cup \{\infty\}}
\newcommand{\Pj}{{\bf P}}
\newcommand{\Fl}{{\cal F}\!\ell}
\newcommand{\fl}{ f\!\ell}
\newcommand{\FF}{ {\cal F}}
\newcommand{\V}{{\cal V}}
\newcommand{\W}{{\cal W}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\trace}{\mbox{trace}\,}
\newcommand{\tr}{\mbox{Tr}}
%%"àÏ‹L†%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
%%"ñd‰º•t'«'˜a'Ï‹L†%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\Condsum}[2]{\sum_{\stackrel{#1}{#2}}}
\newcommand{\Condsum}[2]{\sum_{%
                        \stackrel{\mbox{\tiny$#1$}}%
                                 {\mbox{\tiny$#2$}}}}
%\newcommand{\Condprod}[2]{\prod_{\stackrel{#1}{#2}}}
\newcommand{\Condprod}[2]{\prod_{%
                        \stackrel{\mbox{\tiny$#1$}}%
                                 {\mbox{\tiny$#2$}}}}
%%s—ñ•\Ž¦—p%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bigzerol}{\smash{\hbox{\bg 0}}}
\newcommand{\bigzerou}{\smash{\lower1.2ex\hbox{\bg 0}}}
%%%Display style •ª"•\Ž¦%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dfrac#1#2{{\displaystyle\frac{#1}{#2}}}

%%%}Ž®ì¬—p%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\normalbaselines}{\baselineskip20pt
 \lineskip3pt\lineskiplimit3pt}
%ã"Y'¦Žš''«‰E–îˆó
\newcommand{\mapright}[1]{\smash{\mathop{
 \hbox to 1cm{\rightarrowfill}}\limits^{#1}}}

%‰º"Y'¦Žš''«‰E–îˆó
\newcommand{\maprightb}[1]{\smash{\mathop{
 \hbox to 1cm{\rightarrowfill}}\limits_{#1}}}


%‰º"Y'¦Žš''«¶–îˆó
\newcommand{\mapleft}[1]{\smash{\mathop{
 \hbox to 1cm{\leftarrowfill}}\limits_{#1}}}

%‰E"Y'¦Žš''«ã–îˆó
\newcommand{\mapup}[1]{\Big\uparrow
 \rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}

%¶"Y'¦Žš''«‰º–îˆó
\newcommand{\mapdown}[1]{\Big\downarrow
 \llap{$\vcenter{\hbox{$\scriptstyle#1\,\,\,$}}$}}

%‰E"Y'¦Žš''«‰º–îˆó
\newcommand{\mapdownr}[1]{\Big\downarrow
 \rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
%%%ß'ÌŒ©o'µ%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\section{\@startsection {section}{1}{\z@}{3.5ex plus 1ex minus 
 .2ex}{2.3ex plus .2ex}{\large\bf}}
\makeatother

%%newtheoremŠÂ‹«'̕ύX%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\@begintheorem#1#2{\it \trivlist \item[\hskip \labelsep{\bf #1\ #2.}]}
\def\@opargbegintheorem#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3).}]}
\makeatother
%%%%%'藝‹LqŠÂ‹«%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand {\thesection}{\arabic{section}.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{Thm}{Theorem}[section]
\renewcommand{\theThm}{\thesection\arabic{Thm}}
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Lemma}[Thm]{Lemma}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Fact}[Thm]{Fact}
\newenvironment{Proof}{\rm \hskip -0.5cm(Proof.)\quad}{\hfill (q.e.d.)\vskip .5cm}
\newtheorem{Example}[Thm]{Example}
\newenvironment{Exa}{\begin{Example} \rm}{\end{Example}}
\newtheorem{Remark}[Thm]{Remark}
\newenvironment{Rmk}{\begin{Remark} \rm}{\end{Remark}}
\newtheorem{Definition}[Thm]{Definition}
\newenvironment{Def}{\begin{Definition} \rm}{\end{Definition}}

%%%"Ž®"ԍ†§Œä%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\theequation}{\thesection\arabic{equation}}

\makeatletter
\@addtoreset{equation}{section}
\makeatother

\renewcommand{\labelenumi}{(\arabic{enumi})}
%%%‰Óð''«%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%namelist environment by Nelson H. Beebe
%form: \begin{namelist}{maximal width}
\newcommand{\namelistlabel}[1]{\mbox{#1}\hfil}
\newenvironment{namelist}[1]{%
\begin{list}{}
{\let\makelabel\namelistlabel
\settowidth{\labelwidth}{#1}
\setlength{\leftmargin}{1.1\labelwidth}}
}{%
\end{list}}

